Retina : Low-Power Eye Tracking with Event Camera and Spiking Hardware

This paper introduces a neuromorphic methodology for eye tracking, harnessing pure event data captured by a Dynamic Vision Sensor (DVS) camera. The framework integrates a directly trained Spiking Neuron Network (SNN) regression model and leverages a state-of-the-art low power edge neuromorphic processor - Speck, collectively aiming to advance the precision and efficiency of eye-tracking systems. First, we introduce a representative event-based eye-tracking dataset, "Ini-30", which was collected with two glass-mounted DVS cameras from thirty volunteers. Then,a SNN model, based on Integrate And Fire (IAF) neurons, named "Retina", is described , featuring only 64k parameters (6.63x fewer than the latest) and achieving pupil tracking error of only 3.24 pixels in a 64x64 DVS input. The continous regression output is obtained by means of convolution using a non-spiking temporal 1D filter slided across the output spiking layer. Finally, we evaluate Retina on the neuromorphic processor, showing an end-to-end power between 2.89-4.8 mW and a latency of 5.57-8.01 mS dependent on the time window. We also benchmark our model against the latest event-based eye-tracking method, "3ET", which was built upon event frames. Results show that Retina achieves superior precision with 1.24px less pupil centroid error and reduced computational complexity with 35 times fewer MAC operations. We hope this work will open avenues for further investigation of close-loop neuromorphic solutions and true event-based training pursuing edge performance.

==> sec/5_evaluation.tex <==
% \section{Evaluation metrics}
% \subsection{Precision}
% To train our network, we constructed a bounding box around the original 1-pixel label representing the center location of the pupil and expanded it to 5 pixel in each direction. Our precision results are based on the intersection over union (IoU) of the predicted bounding box w.r.t the target bounding box as well as the actual centroid error in pixels.

% \subsection{Efficiency}
%  We evaluated the efficiency of our algorithm by measuring the power (P) [mW] consumption on the neuromorphic \ac{soc} and by counting the number of parameters and \ac{mac} operations. 
